Trustworthy FinAInce: Unpacking How AI-Mediated Financial Advice is Judged

As generative AI is increasingly used as a source of personal financial guidance, understanding how people appraise such advice is important for supporting appropriate reliance. We conducted a randomized vignette experiment with 285 U.S. adults across eight financial decisions, independently varying three advice styles---AI, expert, and online community---and displayed source labels while holding the underlying recommendation consistent. Advice style most strongly shaped message and safety appraisals, Expert labels selectively increased perceived source knowledge, and decision context primarily shaped risk and safety appraisals. These appraisals were associated with downstream judgments, with models explaining 69.2% of overall quality, 75.9% of trust, and 82.9% of intended reliance. Expert-style advice also remained most preferred when shown without source labels. Our findings have implications for understanding financial advice evaluation, distinguishing the roles of advice style and source labels, and designing financial AI that supports grounded evaluation rather than simply maximizing trust.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.16   Emergency release: fixes a typo in the code.

Version 2.15   Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> tables/11_regression_formulas.tex <==
% Table: Mixed-effects model specifications
\begin{table*}[t]
\centering
\sffamily

\caption{Specification of linear mixed-effects models used in the
advice-evaluation pathway analyses.}
\label{tab:model-specifications}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.35}

\begin{tabular}{
    p{0.30\textwidth}
    p{0.20\textwidth}
    p{0.30\textwidth}
}
\toprule
\textbf{Model}
& \textbf{Outcome}
& \textbf{Specification} \\
\midrule

\multicolumn{3}{l}{\textit{Initial advice appraisals}} \\[0.15em]

Message Appraisal
& Message Appraisal
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\

Risk Acknowledgment
& Risk Acknowledgment
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\

Safety Concern
& Safety Concern
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\

Source Knowledge
& Source Knowledge
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\[0.35em]


\multicolumn{3}{l}{\textit{Overall Quality}} \\[0.15em]

Quality: Upstream
& Overall Quality
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\

Quality: Evaluation-adjusted
& Overall Quality
& $Y = \mathcal{U} + \mathcal{A}
+ (1 \mid \mathrm{Participant})$ \\[0.35em]


\multicolumn{3}{l}{\textit{Trust}} \\[0.15em]

Trust: Upstream
& Trust
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\

Trust: Evaluation-adjusted
& Trust
& $Y = \mathcal{U} + \mathcal{A}
+ \mathrm{Overall\ Quality}
+ (1 \mid \mathrm{Participant})$ \\[0.35em]


\multicolumn{3}{l}{\textit{Reliance}} \\[0.15em]

Reliance: Upstream
& Reliance
& $Y = \mathcal{U} + (1 \mid \mathrm{Participant})$ \\

Reliance: Evaluation-adjusted
& Reliance
& $Y = \mathcal{U} + \mathcal{A}
+ \mathrm{Overall\ Quality}
+ \mathrm{Trust}
+ (1 \mid \mathrm{Participant})$ \\

\bottomrule
\end{tabular}

\vspace{0.5em}
\begin{minipage}{0.96\textwidth}
\footnotesize
\textit{Note.}
All models are linear mixed-effects models with a participant-level
random intercept.

$\mathcal{U}$ denotes the common upstream predictor set:
advice communication style (Expert and Online Community [OC], with AI
as the reference), displayed source attribution (AI, Expert, and OC,
with Unlabeled as the reference), stakes (high vs.\ low), external
uncertainty (high vs.\ low), verifiability (high vs.\ low), and
standardized scenario familiarity.
\[\mathcal{U} =
\text{Advice Style}
+ \text{Displayed Label}
+ \text{Stakes}
+ \text{External Uncertainty}
+ \text{Verifiability}
+ \text{Scenario Familiarity}
\]
$\mathcal{A}$ denotes the four intermediate advice-evaluation variables:
standardized Message Appraisal, Risk Acknowledgment, Safety Concern,
and Source Knowledge.

\[
\mathcal{A} =
\text{Message Appraisal}
+ \text{Risk Acknowledgement}
+ \text{Safety Concern}
+ \text{Source Knowledge}
\]

All outcome variables were standardized prior to estimation.
The appraisal-adjusted and evaluation-adjusted models were specified
sequentially to examine whether associations of upstream design factors
with downstream judgments were attenuated after accounting for
participants' evaluations. These models characterize statistical
associations and are not interpreted as causal mediation.
\end{minipage}

\end{table*}

==> tables/12_full_appraisal.tex <==
% Appendix Table: Full initial appraisal models
\begin{table*}[t]
\centering
\sffamily

\caption{Full mixed-effects models predicting initial advice appraisals.}
\label{tab:appraisal-models-full}

\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{lcccc}
\toprule
\textbf{Predictor}
& \makecell{\textbf{Message}\\\textbf{Appraisal}}
& \makecell{\textbf{Risk}\\\textbf{Acknowledgement}}
& \makecell{\textbf{Safety}\\\textbf{Concern}}
& \makecell{\textbf{Source}\\\textbf{Knowledge}} \\
\midrule

\multicolumn{5}{l}{\textit{Advice communication style}} \\

Expert vs.\ AI
& $0.334^{***}$ $(0.059)$
& $-0.061$ $(0.064)$
& $-0.245^{***}$ $(0.057)$
& $0.141^{*}$ $(0.063)$ \\

OC vs.\ AI
& $0.223^{***}$ $(0.059)$
& $-0.147^{*}$ $(0.064)$
& $-0.127^{*}$ $(0.057)$
& $-0.174^{**}$ $(0.063)$ \\[0.2em]

\multicolumn{5}{l}{\textit{Displayed source attribution}} \\

AI label vs.\ Unlabeled
& $0.075$ $(0.090)$
& $-0.088$ $(0.095)$
& $-0.141$ $(0.098)$
& $0.049$ $(0.094)$ \\

Expert label vs.\ Unlabeled
& $0.190^{*}$ $(0.090)$
& $-0.026$ $(0.095)$
& $-0.166$ $(0.098)$
& $0.225^{*}$ $(0.094)$ \\

OC label vs.\ Unlabeled
& $0.168$ $(0.089)$
& $-0.044$ $(0.093)$
& $-0.119$ $(0.097)$
& $0.091$ $(0.093)$ \\[0.2em]

\multicolumn{5}{l}{\textit{Decision context}} \\

High stakes
& $-0.241^{***}$ $(0.048)$
& $0.083$ $(0.052)$
& $0.436^{***}$ $(0.046)$
& $0.010$ $(0.051)$ \\

High external uncertainty
& $-0.072$ $(0.046)$
& $0.310^{***}$ $(0.050)$
& $0.026$ $(0.044)$
& $-0.005$ $(0.049)$ \\

High verifiability
& $0.099$ $(0.075)$
& $-0.199^{*}$ $(0.078)$
& $-0.292^{***}$ $(0.084)$
& $0.036$ $(0.077)$ \\

Scenario familiarity
& $0.319^{***}$ $(0.029)$
& $0.140^{***}$ $(0.031)$
& $-0.125^{***}$ $(0.029)$
& $0.206^{***}$ $(0.031)$ \\

\midrule

$R^2_m$
& .170 & .054 & .115 & .067 \\

$R^2_c$
& .405 & .298 & .458 & .312 \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.98\textwidth}
\footnotesize
\textit{Note.}
Cells report standardized fixed-effect coefficients with standard
errors in parentheses. Models include participant-level random
intercepts. AI-style advice and the unlabeled condition are reference
categories. $N=1{,}140$ evaluations from 285 participants.
$R^2_m$ and $R^2_c$ denote marginal and conditional Nakagawa-style
$R^2$, respectively. Higher Safety Concern indicates greater perceived
financial harm or misleadingness.
$^{*}p<.05$, $^{**}p<.01$, $^{***}p<.001$.
\end{minipage}

\end{table*}

==> tables/13_full_downstream.tex <==
% Appendix Table: Full downstream nested models
\begin{table*}[t]
\centering
\sffamily

\caption{Full upstream and evaluation-adjusted mixed-effects models
for Overall Quality, Trust, and Intended Reliance.}
\label{tab:downstream-models-full}

\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.18}
\scriptsize

\begin{tabular}{lcccccc}
\toprule
&
\multicolumn{2}{c}{\textbf{Overall Quality}}
&
\multicolumn{2}{c}{\textbf{Trust}}
&
\multicolumn{2}{c}{\textbf{Reliance}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}

\textbf{Predictor}
& \textbf{Upstream}
& \textbf{Adjusted}
& \textbf{Upstream}
& \textbf{Adjusted}
& \textbf{Upstream}
& \textbf{Adjusted} \\
\midrule

\multicolumn{7}{l}{\textit{Advice communication style}} \\

Expert vs.\ AI
& $.205^{***}$ (.060)
& $.011$ (.039)
& $.185^{**}$ (.061)
& $-.028$ (.035)
& $.173^{**}$ (.061)
& $-.019$ (.031) \\

OC vs.\ AI
& $-.004$ (.060)
& $.005$ (.039)
& $.009$ (.062)
& $-.009$ (.035)
& $.023$ (.061)
& $.002$ (.032) \\[0.15em]

\multicolumn{7}{l}{\textit{Displayed source attribution}} \\

AI label vs.\ Unlabeled
& $.126$ (.094)
& $.074$ (.051)
& $.066$ (.092)
& $-.038$ (.045)
& $.103$ (.090)
& $.029$ (.035) \\

Expert label vs.\ Unlabeled
& $.248^{**}$ (.094)
& $.064$ (.051)
& $.176$ (.092)
& $-.046$ (.045)
& $.210^{*}$ (.090)
& $.013$ (.035) \\

OC label vs.\ Unlabeled
& $.170$ (.093)
& $.060$ (.050)
& $.154$ (.091)
& $.004$ (.044)
& $.189^{*}$ (.089)
& $.040$ (.034) \\[0.15em]

\multicolumn{7}{l}{\textit{Decision context}} \\

High stakes
& $-.040$ (.049)
& $.069^{*}$ (.032)
& $-.107^{*}$ (.050)
& $-.000$ (.029)
& $-.155^{**}$ (.050)
& $-.048$ (.026) \\

High external uncertainty
& $-.013$ (.047)
& $-.008$ (.031)
& $.001$ (.048)
& $.014$ (.028)
& $.017$ (.048)
& $.030$ (.025) \\

High verifiability
& $.152$ (.079)
& $.091^{*}$ (.041)
& $.166^{*}$ (.076)
& $.026$ (.036)
& $.178^{*}$ (.074)
& $.022$ (.025) \\

Scenario familiarity
& $.256^{***}$ (.030)
& $.038^{*}$ (.019)
& $.280^{***}$ (.030)
& $.040^{*}$ (.017)
& $.324^{***}$ (.030)
& $.049^{***}$ (.014) \\[0.15em]

\multicolumn{7}{l}{\textit{Evaluation pathway}} \\

Message Appraisal
& ---
& $.325^{***}$ (.024)
& ---
& $.132^{***}$ (.023)
& ---
& $.079^{***}$ (.020) \\

Risk Acknowledgement
& ---
& $.075^{***}$ (.019)
& ---
& $.024$ (.017)
& ---
& $-.015$ (.014) \\

Safety Concern
& ---
& $-.088^{***}$ (.019)
& ---
& $-.125^{***}$ (.018)
& ---
& $-.050^{***}$ (.014) \\

Source Knowledge
& ---
& $.489^{***}$ (.022)
& ---
& $.109^{***}$ (.024)
& ---
& $.047^{*}$ (.020) \\

Overall Quality
& ---
& ---
& ---
& $.607^{***}$ (.027)
& ---
& $.206^{***}$ (.027) \\

Trust
& ---
& ---
& ---
& ---
& ---
& $.594^{***}$ (.025) \\

\midrule

$R^2_m$
& .098 & .692
& .112 & .759
& .148 & .829 \\

$R^2_c$
& .373 & .742
& .351 & .795
& .362 & .829 \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.98\textwidth}
\footnotesize
\textit{Note.}
Cells report standardized fixed-effect coefficients with standard
errors in parentheses. Upstream models include communication style,
displayed source attribution, decision-context variables, and scenario
familiarity. Adjusted models additionally introduce appraisal variables;
Overall Quality is further included in the Trust model, and Overall
Quality and Trust are further included in the Reliance model.
All models include participant-level random intercepts.
$N=1{,}140$ evaluations from 285 participants.
$R^2_m$ and $R^2_c$ denote marginal and conditional Nakagawa-style
$R^2$, respectively.
$^{*}p<.05$, $^{**}p<.01$, $^{***}p<.001$.
\end{minipage}

\end{table*}

==> tables/14_bootstrap_table.tex <==
\begin{table*}[t]
\centering
\sffamily


\caption{
Bootstrap decomposition of appraisal-carried pathways from advice style
and source labels to intended Reliance.
Bolded estimates have 95\% bootstrap confidence intervals excluding zero.
\textcolor{red}{[can move to appendix]}}
\label{tab:pathway_decomposition}

\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.18}

\begin{tabular}{lccccc}
\toprule
\textbf{Upstream contrast}
& \makecell{\textbf{Message}\\\textbf{Appraisal}}
& \makecell{\textbf{Risk}\\\textbf{Ack.}}
& \makecell{\textbf{Safety}\\\textbf{Concern}}
& \makecell{\textbf{Source}\\\textbf{Knowledge}}
& \textbf{Total} \\
\midrule

\multicolumn{6}{l}{\textit{Advice style}} \\

Expert vs.\ AI
& \makecell{\textbf{.114}\\\textbf{[.069,.166]}}
& \makecell{-.003\\{}[-.009,.002]}
& \makecell{\textbf{.043}\\\textbf{[.023,.068]}}
& \makecell{\textbf{.055}\\\textbf{[.009,.106]}}
& \makecell{\textbf{.210}\\\textbf{[.115,.309]}} \\[0.50em]

OC vs.\ AI
& \makecell{\textbf{.076}\\\textbf{[.033,.123]}}
& \makecell{-.006\\{}[-.017,.001]}
& \makecell{\textbf{.022}\\\textbf{[.003,.045]}}
& \makecell{\textbf{-.068}\\\textbf{[-.129,-.014]}}
& \makecell{.023\\{}[-.083,.129]} \\[0.35em]

\midrule
\multicolumn{6}{l}{\textit{Source labels}} \\

AI vs.\ Unlabeled
& \makecell{.025\\{}[-.033,.090]}
& \makecell{-.003\\{}[-.014,.004]}
& \makecell{.024\\{}[-.009,.061]}
& \makecell{.018\\{}[-.053,.095]}
& \makecell{.064\\{}[-.072,.209]} \\[0.50em]

Expert vs.\ Unlabeled
& \makecell{\textbf{.064}\\\textbf{[.001,.129]}}
& \makecell{-.001\\{}[-.011,.008]}
& \makecell{.028\\{}[-.006,.066]}
& \makecell{\textbf{.088}\\\textbf{[.014,.164]}}
& \makecell{\textbf{.179}\\\textbf{[.032,.325]}} \\[0.50em]

OC vs.\ Unlabeled
& \makecell{\textbf{.058}\\\textbf{[.001,.118]}}
& \makecell{-.002\\{}[-.011,.006]}
& \makecell{.020\\{}[-.015,.056]}
& \makecell{.038\\{}[-.036,.114]}
& \makecell{.114\\{}[-.022,.256]} \\[0.50em]

\bottomrule
\end{tabular}

\vspace{0.3em}
\parbox{0.96\textwidth}{
\scriptsize
\textit{Note.}
Cells report bootstrap mean pathway estimates with 95\% percentile confidence intervals
from 2,000 participant-level bootstrap samples.
AI is the reference for advice style; Unlabeled is the reference for source labels.
Positive values indicate pathways toward greater intended Reliance.
These estimates are statistical pathway decompositions rather than causal mediation effects.
}
\end{table*}

==> tables/15_full_reliance_bootstrap.tex <==
\begin{table*}[t]
\centering
\sffamily
\scriptsize

\caption{
Full route-level bootstrap decomposition of appraisal-carried pathways
to Reliance. Values are bootstrap mean pathway estimates with 95\%
percentile confidence intervals.
}
\label{tab:reliance_pathways_full}

\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.15\textwidth}
    p{0.15\textwidth}
    c c c c c
}
\toprule
\textbf{Contrast}
& \textbf{Appraisal}
& \textbf{Appraisal only}
& \textbf{Via Quality}
& \textbf{Via Trust}
& \textbf{Via Quality$\rightarrow$Trust}
& \textbf{Total} \\
\midrule

\multicolumn{7}{l}{\textit{Expert style vs.\ AI}} \\

& Message Appraisal
& .027 [.010, .048]
& .023 [.011, .039]
& .026 [.012, .043]
& .039 [.022, .059]
& .114 [.069, .166] \\

& Risk Acknowledgment
& .001 [-.001, .005]
& -.001 [-.003, .001]
& -.001 [-.004, .001]
& -.002 [-.005, .001]
& -.003 [-.009, .002] \\

& Safety Concern
& .013 [.005, .023]
& .004 [.002, .009]
& .018 [.009, .030]
& .008 [.003, .014]
& .043 [.023, .068] \\

& Source Knowledge
& .007 [-.001, .019]
& .014 [.002, .030]
& .009 [.001, .021]
& .025 [.004, .051]
& .055 [.009, .106] \\

& \textit{All appraisals}
& ---
& ---
& ---
& ---
& .210 [.115, .309] \\

\midrule

\multicolumn{7}{l}{\textit{OC style vs.\ AI}} \\

& Message Appraisal
& .018 [.005, .034]
& .015 [.006, .028]
& .017 [.006, .032]
& .026 [.010, .044]
& .076 [.033, .123] \\

& Risk Acknowledgment
& .002 [-.002, .008]
& -.002 [-.006, -.000]
& -.002 [-.007, .001]
& -.004 [-.009, -.000]
& -.006 [-.017, .001] \\

& Safety Concern
& .006 [.000, .015]
& .002 [.000, .005]
& .009 [.001, .020]
& .004 [.000, .010]
& .022 [.003, .045] \\

& Source Knowledge
& -.008 [-.024, .001]
& -.018 [-.036, -.003]
& -.011 [-.025, -.002]
& -.031 [-.060, -.006]
& -.068 [-.129, -.014] \\

& \textit{All appraisals}
& ---
& ---
& ---
& ---
& .023 [-.083, .129] \\

\midrule

\multicolumn{7}{l}{\textit{AI label vs.\ Unlabeled}} \\

& Message Appraisal
& .006 [-.008, .023]
& .005 [-.007, .019]
& .006 [-.008, .023]
& .008 [-.012, .029]
& .025 [-.033, .090] \\

& Risk Acknowledgment
& .001 [-.002, .006]
& -.001 [-.005, .001]
& -.001 [-.005, .002]
& -.002 [-.008, .002]
& -.003 [-.014, .004] \\

& Safety Concern
& .007 [-.003, .019]
& .002 [-.001, .007]
& .010 [-.004, .026]
& .004 [-.002, .012]
& .024 [-.009, .061] \\

& Source Knowledge
& .002 [-.007, .015]
& .005 [-.014, .025]
& .003 [-.009, .018]
& .008 [-.024, .042]
& .018 [-.053, .095] \\

& \textit{All appraisals}
& ---
& ---
& ---
& ---
& .064 [-.072, .209] \\

\midrule

\multicolumn{7}{l}{\textit{Expert label vs.\ Unlabeled}} \\

& Message Appraisal
& .015 [.000, .038]
& .013 [.000, .027]
& .015 [.000, .034]
& .022 [.000, .045]
& .064 [.001, .129] \\

& Risk Acknowledgment
& .000 [-.004, .005]
& -.000 [-.003, .003]
& -.000 [-.004, .003]
& -.001 [-.006, .005]
& -.001 [-.011, .008] \\

& Safety Concern
& .008 [-.002, .021]
& .003 [-.001, .008]
& .012 [-.003, .029]
& .005 [-.001, .014]
& .028 [-.006, .066] \\

& Source Knowledge
& .011 [-.001, .033]
& .022 [.004, .045]
& .015 [.002, .034]
& .039 [.006, .077]
& .088 [.014, .164] \\

& \textit{All appraisals}
& ---
& ---
& ---
& ---
& .179 [.032, .325] \\

\midrule

\multicolumn{7}{l}{\textit{OC label vs.\ Unlabeled}} \\

& Message Appraisal
& .014 [.000, .032]
& .011 [.000, .025]
& .013 [.000, .031]
& .020 [.000, .041]
& .058 [.001, .118] \\

& Risk Acknowledgment
& .001 [-.003, .005]
& -.001 [-.004, .002]
& -.001 [-.004, .002]
& -.001 [-.006, .004]
& -.002 [-.011, .006] \\

& Safety Concern
& .006 [-.005, .018]
& .002 [-.001, .007]
& .008 [-.006, .024]
& .004 [-.003, .012]
& .020 [-.015, .056] \\

& Source Knowledge
& .005 [-.004, .019]
& .010 [-.009, .032]
& .006 [-.006, .022]
& .017 [-.016, .053]
& .038 [-.036, .114] \\

& \textit{All appraisals}
& ---
& ---
& ---
& ---
& .114 [-.022, .256] \\

\bottomrule
\end{tabular}

\vspace{0.3em}
\parbox{0.97\textwidth}{
\footnotesize
\textit{Note.}
``Appraisal only'' denotes
$X\rightarrow A\rightarrow Reliance$.
The remaining columns correspond to
$X\rightarrow A\rightarrow Quality\rightarrow Reliance$,
$X\rightarrow A\rightarrow Trust\rightarrow Reliance$, and
$X\rightarrow A\rightarrow Quality\rightarrow Trust\rightarrow Reliance$,
respectively.
}

\end{table*}

==> tables/16_full_trust_bootstrap.tex <==
\begin{table*}[t]
\centering
\sffamily
\scriptsize

\caption{
Parallel bootstrap decomposition with Trust as the terminal outcome.
Values are bootstrap mean pathway estimates with 95\% percentile
confidence intervals from 2,000 participant-level bootstrap samples.
}
\label{tab:trust_pathways}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.15\textwidth}
    p{0.15\textwidth}
    c c c
}
\toprule
\textbf{Contrast}
& \textbf{Appraisal}
& \textbf{Appraisal only}
& \textbf{Via Quality}
& \textbf{Total} \\
\midrule

\multicolumn{5}{l}{\textit{Expert style vs.\ AI}} \\

& Message Appraisal
& .044 [.021, .074]
& .066 [.038, .100]
& .110 [.066, .160] \\

& Risk Acknowledgment
& -.002 [-.006, .001]
& -.003 [-.009, .002]
& -.004 [-.014, .003] \\

& Safety Concern
& .031 [.016, .049]
& .013 [.005, .024]
& .044 [.024, .069] \\

& Source Knowledge
& .015 [.002, .035]
& .042 [.007, .084]
& .058 [.010, .112] \\

& \textit{All appraisals}
& ---
& ---
& .207 [.111, .309] \\

\midrule

\multicolumn{5}{l}{\textit{OC style vs.\ AI}} \\

& Message Appraisal
& .029 [.010, .055]
& .044 [.018, .074]
& .073 [.031, .121] \\

& Risk Acknowledgment
& -.004 [-.011, .001]
& -.007 [-.016, -.001]
& -.011 [-.024, -.001] \\

& Safety Concern
& .016 [.002, .032]
& .007 [.001, .016]
& .023 [.002, .045] \\

& Source Knowledge
& -.019 [-.041, -.003]
& -.052 [-.099, -.011]
& -.071 [-.132, -.015] \\

& \textit{All appraisals}
& ---
& ---
& .013 [-.095, .124] \\

\midrule

\multicolumn{5}{l}{\textit{AI label vs.\ Unlabeled}} \\

& Message Appraisal
& .010 [-.013, .040]
& .014 [-.019, .049]
& .024 [-.032, .086] \\

& Risk Acknowledgment
& -.002 [-.009, .003]
& -.004 [-.013, .004]
& -.006 [-.020, .007] \\

& Safety Concern
& .017 [-.007, .044]
& .007 [-.003, .021]
& .024 [-.010, .061] \\

& Source Knowledge
& .005 [-.015, .030]
& .014 [-.041, .070]
& .019 [-.054, .097] \\

& \textit{All appraisals}
& ---
& ---
& .062 [-.080, .213] \\

\midrule

\multicolumn{5}{l}{\textit{Expert label vs.\ Unlabeled}} \\

& Message Appraisal
& .025 [.000, .057]
& .037 [.001, .075]
& .062 [.001, .124] \\

& Risk Acknowledgment
& -.001 [-.006, .005]
& -.001 [-.010, .008]
& -.002 [-.016, .012] \\

& Safety Concern
& .020 [-.004, .049]
& .008 [-.002, .022]
& .029 [-.007, .067] \\

& Source Knowledge
& .025 [.003, .056]
& .067 [.011, .127]
& .091 [.015, .170] \\

& \textit{All appraisals}
& ---
& ---
& .180 [.030, .328] \\

\midrule

\multicolumn{5}{l}{\textit{OC label vs.\ Unlabeled}} \\

& Message Appraisal
& .022 [.000, .052]
& .033 [.001, .068]
& .055 [.001, .113] \\

& Risk Acknowledgment
& -.001 [-.007, .004]
& -.002 [-.010, .007]
& -.003 [-.016, .010] \\

& Safety Concern
& .014 [-.011, .041]
& .006 [-.004, .019]
& .020 [-.015, .057] \\

& Source Knowledge
& .011 [-.010, .037]
& .029 [-.027, .091]
& .039 [-.036, .121] \\

& \textit{All appraisals}
& ---
& ---
& .112 [-.029, .258] \\

\bottomrule
\end{tabular}

\vspace{0.3em}
\parbox{0.97\textwidth}{
\footnotesize
\textit{Note.}
For Trust, each appraisal contributes through two modeled routes:
$X\rightarrow A\rightarrow Trust$ and
$X\rightarrow A\rightarrow Quality\rightarrow Trust$.
The qualitative pattern closely mirrors the Reliance-terminal decomposition.
}

\end{table*}

==> tables/17_Contrast_tables.tex <==
\begin{table}[t]
\centering
\sffamily
\footnotesize


\caption{
Bootstrap contrasts comparing the Message Appraisal and Source Knowledge
pathways to intended Reliance.
}
\label{tab:pathway_contrasts}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{
    p{0.45\columnwidth}
    c
    c
}
\toprule
\textbf{Pathway contrast}
& \textbf{Estimate}
& \textbf{95\% CI} \\
\midrule

\multicolumn{3}{l}{\textit{Expert}} \\

Expert style:
\textit{Message Appraisal} $-$ \textit{Source Knowledge}
& \textbf{.060}
& \textbf{[.006, .112]} \\

Expert label:
\textit{Message Appraisal} $-$ \textit{Source Knowledge}
& -.021
& [-.081, .035] \\

Style--label contrast-of-contrasts
& \textbf{.081}
& \textbf{[.014, .148]} \\

\midrule

\multicolumn{3}{l}{\textit{Online Community}} \\

OC style:
\textit{Message Appraisal} $-$ \textit{Source Knowledge}
& \textbf{.144}
& \textbf{[.101, .190]} \\

OC label:
\textit{Message Appraisal} $-$ \textit{Source Knowledge}
& .020
& [-.043, .082] \\

Style--label contrast-of-contrasts
& \textbf{.124}
& \textbf{[.045, .212]} \\

\bottomrule
\end{tabular}

\vspace{0.3em}
\parbox{0.95\columnwidth}{
\footnotesize
\textit{Note.}
Positive values indicate a relatively stronger \textit{Message Appraisal} pathway
than \textit{Source Knowledge} pathway.
The contrast-of-contrasts compares this relative pathway strength
between advice style and source labels.
Bolded intervals exclude zero.
}

\end{table}

==> tables/18_likelihood_ratio_test.tex <==
\begin{table}[t]
\sffamily
\centering

\caption{
Likelihood-ratio tests comparing additive mixed-effects models with
models including the Advice Style $\times$ Displayed Label interaction.
The interaction added six fixed-effect parameters in each model.
}
\label{tab:style-label-interactions}

\begin{tabular}{lrr}
\toprule
\textbf{Outcome}
& $\boldsymbol{\chi^2(6)}$
& $\boldsymbol{p}$ \\
\midrule

Message Appraisal       & 3.71 & .716 \\
Risk Acknowledgement    & 7.32 & .293 \\
Safety Concern          & 2.20 & .901 \\
Source Knowledge        & 3.29 & .772 \\
Overall Quality         & 4.83 & .566 \\
Trust                   & 1.48 & .961 \\
Reliance                & 2.17 & .904 \\

\bottomrule
\end{tabular}
\end{table}

==> tables/19_simple_effects_labels_styles.tex <==
% Requires only booktabs (already common in acmart/CHI templates).
% Each cell shows beta followed by the Benjamini--Hochberg FDR-adjusted p-value in parentheses.
% Significant cells (adjusted p < .05) are bolded.

% ------------------------------------------------------------
% Appendix Table A6: label effects within communication style
% ------------------------------------------------------------
\begin{table*}[t]
\centering
\sffamily
\caption{Displayed-label effects within each communication style. Each cell reports the standardized fixed-effect contrast $\beta$ relative to the \textit{No label} condition, followed by the Benjamini--Hochberg FDR-adjusted $p$-value in parentheses. Bold cells indicate adjusted $p<.05$.}
\label{tab:label-within-style-matrix}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.10}

\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(a) Message Appraisal}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $0.151\;(.384)$ & $0.068\;(.926)$ & $0.248\;(.295)$ \\
Expert & $0.042\;(.926)$ & $0.171\;(.353)$ & $0.014\;(.926)$ \\
OC & $-0.034\;(.926)$ & $0.309\;(.295)$ & $0.210\;(.295)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(b) Risk Acknowledgement}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $0.052\;(.879)$ & $0.169\;(.534)$ & $0.011\;(.988)$ \\
Expert & $-0.214\;(.534)$ & $0.002\;(.988)$ & $0.094\;(.825)$ \\
OC & $-0.169\;(.534)$ & $-0.278\;(.534)$ & $-0.196\;(.534)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(c) Safety Concern}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $-0.102\;(.548)$ & $-0.153\;(.507)$ & $-0.280\;(.507)$ \\
Expert & $-0.218\;(.507)$ & $-0.145\;(.507)$ & $-0.089\;(.642)$ \\
OC & $-0.163\;(.507)$ & $-0.227\;(.507)$ & $-0.055\;(.664)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(d) Source Knowledge}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $0.029\;(.941)$ & $0.102\;(.939)$ & $0.012\;(.941)$ \\
Expert & $-0.071\;(.941)$ & $0.206\;(.327)$ & $0.026\;(.941)$ \\
OC & $0.165\;(.687)$ & $0.358\;(.252)$ & $0.204\;(.327)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(e) Overall Quality}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $0.221\;(.182)$ & $0.278\;(.182)$ & $0.363\;(.091)$ \\
Expert & $0.124\;(.647)$ & $0.292\;(.091)$ & $0.070\;(.733)$ \\
OC & $-0.002\;(.990)$ & $0.107\;(.647)$ & $0.085\;(.647)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(f) Trust}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $0.093\;(.637)$ & $0.194\;(.480)$ & $0.247\;(.480)$ \\
Expert & $0.107\;(.637)$ & $0.164\;(.480)$ & $0.038\;(.902)$ \\
OC & $0.001\;(.995)$ & $0.156\;(.591)$ & $0.159\;(.480)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(g) Reliance}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Style} & \textbf{AI label} & \textbf{Expert label} & \textbf{OC label} \\
\midrule
AI & $0.167\;(.312)$ & $0.193\;(.313)$ & $0.269\;(.311)$ \\
Expert & $-0.019\;(.904)$ & $0.169\;(.312)$ & $0.058\;(.785)$ \\
OC & $0.122\;(.553)$ & $0.255\;(.311)$ & $0.228\;(.311)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\vspace{0.15em}
\begin{minipage}{0.98\textwidth}
\footnotesize
\textit{Note.} All coefficients are relative to the \textit{No label} condition. Positive coefficients indicate higher ratings under the displayed label than under no label; negative coefficients indicate lower ratings. Values in parentheses are Benjamini--Hochberg FDR-adjusted $p$-values. FDR correction was applied across the nine label-within-style contrasts for each outcome.
\end{minipage}
\end{table*}

% ------------------------------------------------------------
% Appendix Table A7: style effects within displayed label
% ------------------------------------------------------------
\begin{table*}[t]
\centering
\sffamily
\caption{Communication-style effects within each displayed-label condition. Each cell reports the standardized fixed-effect contrast $\beta$, followed by the Benjamini--Hochberg FDR-adjusted $p$-value in parentheses. Bold cells indicate adjusted $p<.05$.}
\label{tab:style-within-label-matrix}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.10}

\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(a) Message Appraisal}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $\mathbf{0.390\;(.001)}$ & $0.226\;(.082)$ & $0.164\;(.213)$ \\
AI label & $0.281\;(.157)$ & $0.041\;(.864)$ & $0.240\;(.296)$ \\
Expert label & $\mathbf{0.493\;(.006)}$ & $\mathbf{0.467\;(.032)}$ & $0.026\;(.864)$ \\
OC label & $0.156\;(.482)$ & $0.188\;(.302)$ & $-0.032\;(.864)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(b) Risk Acknowledgement}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $0.015\;(.889)$ & $0.052\;(.792)$ & $-0.037\;(.803)$ \\
AI label & $-0.251\;(.390)$ & $-0.169\;(.576)$ & $-0.082\;(.792)$ \\
Expert label & $-0.152\;(.576)$ & $-0.396\;(.390)$ & $0.243\;(.390)$ \\
OC label & $0.097\;(.792)$ & $-0.156\;(.576)$ & $0.253\;(.390)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(c) Safety Concern}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $-0.256\;(.092)$ & $-0.147\;(.404)$ & $-0.109\;(.450)$ \\
AI label & $-0.373\;(.120)$ & $-0.209\;(.445)$ & $-0.164\;(.501)$ \\
Expert label & $-0.248\;(.404)$ & $-0.221\;(.450)$ & $-0.028\;(.862)$ \\
OC label & $-0.066\;(.782)$ & $0.077\;(.744)$ & $-0.143\;(.501)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(d) Source Knowledge}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $0.137\;(.399)$ & $\mathbf{-0.295\;(.041)}$ & $\mathbf{0.432\;(<.001)}$ \\
AI label & $0.037\;(.831)$ & $-0.160\;(.467)$ & $0.196\;(.467)$ \\
Expert label & $0.241\;(.303)$ & $-0.040\;(.831)$ & $0.280\;(.290)$ \\
OC label & $0.151\;(.534)$ & $-0.103\;(.609)$ & $0.254\;(.290)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(e) Overall Quality}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $0.277\;(.079)$ & $0.140\;(.372)$ & $0.137\;(.372)$ \\
AI label & $0.180\;(.437)$ & $-0.082\;(.715)$ & $0.263\;(.372)$ \\
Expert label & $0.291\;(.245)$ & $-0.031\;(.928)$ & $0.321\;(.245)$ \\
OC label & $-0.016\;(.928)$ & $-0.137\;(.555)$ & $0.121\;(.564)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(f) Trust}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $0.229\;(.329)$ & $0.049\;(.954)$ & $0.181\;(.359)$ \\
AI label & $0.244\;(.359)$ & $-0.043\;(.954)$ & $0.287\;(.359)$ \\
Expert label & $0.200\;(.453)$ & $0.010\;(.954)$ & $0.189\;(.453)$ \\
OC label & $0.021\;(.954)$ & $-0.039\;(.954)$ & $0.060\;(.954)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\begin{minipage}[t]{0.485\textwidth}
\centering
\textit{(g) Reliance}\\[0.25em]
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Displayed label} & \textbf{Expert--AI} & \textbf{OC--AI} & \textbf{Expert--OC} \\
\midrule
No label & $0.261\;(.141)$ & $0.031\;(.929)$ & $0.229\;(.175)$ \\
AI label & $0.075\;(.929)$ & $-0.014\;(.945)$ & $0.089\;(.929)$ \\
Expert label & $0.237\;(.467)$ & $0.094\;(.929)$ & $0.143\;(.929)$ \\
OC label & $0.049\;(.929)$ & $-0.010\;(.945)$ & $0.060\;(.929)$ \\
\bottomrule
\end{tabular}
\end{minipage}
\par\vspace{0.8em}
\vspace{0.15em}
\begin{minipage}{0.98\textwidth}
\footnotesize
\textit{Note.} Positive coefficients favor the first-named communication style in each column header; negative coefficients favor the second-named style. Values in parentheses are Benjamini--Hochberg FDR-adjusted $p$-values. FDR correction was applied across the twelve style-within-label contrasts for each outcome. These simple contrasts characterize individual source--label cells and should not be interpreted as evidence of moderation in the absence of a significant omnibus Style $\times$ Label interaction.
\end{minipage}
\end{table*}


==> tables/1_participant_demographics.tex <==
% Table: Participant demographics and background characteristics
\begin{table*}[t]
\sffamily

\centering
\caption{Participant demographics and background characteristics.
Continuous variables are reported as mean (SD); categorical variables
are reported as $n$ (\%).}
\label{tab:participant_demographics}

\begin{tabular}{
    p{0.30\textwidth}
    p{0.40\textwidth}
    p{0.30\textwidth}
}
\toprule
\textbf{Characteristic}
& \textbf{Final analytic sample}
& \textbf{Measure source} \\
\midrule

Sample size
& 285
& --- \\

Age
& 39.76 (SD = 12.22)
& --- \\

Gender
& Male: 143 (50.2\%); Female: 137 (48.1\%);
Prefer not to say: 3 (1.1\%); Missing: 2 (0.7\%).
& --- \\

Household income
& Median category: \$50,000--\$74,999.
& --- \\

Financial literacy (0--3)
& 2.66 (SD = 0.68)
& "Big Three"~\cite{lusardiFinancialLiteracyWorld2011, lusardiEconomicImportanceFinancial2014} \\

Self-rated financial literacy
& Very low: 2 (0.7\%); Low: 20 (7.0\%);
Moderate: 154 (54.0\%); High: 90 (31.6\%);
Very high: 19 (6.7\%).
& --- \\

Financial risk tolerance (1--4)
& No financial risks [1]: 36 (12.6\%);
Average risks [2]: 161 (56.5\%);
Above-average risks [3]: 77 (27.0\%);
Substantial risks [4]: 11 (3.9\%).
& SCF item~\cite{grableAssessingConcurrentValidity2001} \\

AI use frequency
& Never: 9 (3.2\%); Rarely: 20 (7.0\%);
Occasionally: 42 (14.7\%);
Regularly: 80 (28.1\%);
Frequently: 134 (47.0\%).
& --- \\

AI use for personal finance
& No, and have not considered it: 53 (18.6\%);
No, but have considered it: 43 (15.1\%);
Yes, once or twice: 102 (35.8\%);
Yes, multiple times: 87 (30.5\%).
& --- \\

Used AI for finance at least once
& 189 (66.3\%)
& --- \\

General trust in AI (1--7)
& 4.63 (SD = 1.50)
& S-TIAS~\cite{mcgrathMeasuringTrustArtificial2025} \\

Human trust propensity (1--7)
& 4.61 (SD = 1.44)
& Propensity to Trust Scale~\cite{frazierDevelopmentValidationPropensity2013} \\

Perceived AI literacy (1--7)
& 5.16 (SD = 0.99)
& PAILQ-6~\cite{grassiniPsychometricValidationPAILQ62024} \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/20_ind_moderator_main.tex <==
\begin{table*}[t]
\sffamily
\centering
\scriptsize
\caption{
Individual differences in trust formation and reliance.
Interaction coefficients are from participant random-intercept
mixed-effects models. Simple slopes report the corresponding association
at one standard deviation below the moderator mean, at the mean, and one
standard deviation above the mean.
}
\label{tab:individual-moderators}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.30}

\begin{tabular}{
    p{0.13\textwidth}
    p{0.18\textwidth}
    p{0.21\textwidth}
    c
    c
    c
    c
    c
    c
}
\toprule
\textbf{Stage}
& \textbf{Moderator}
& \textbf{Moderated association}
& $\boldsymbol{\beta_{\mathrm{int}}}$
& \textbf{95\% CI}
& $\boldsymbol{p_{\mathrm{FDR}}}$
& \multicolumn{3}{c}{\textbf{Simple slope}} \\
\cmidrule(lr){7-9}
&
&
&
&
&
&
$\boldsymbol{-1}$ \textbf{SD}
& \textbf{Mean}
& $\boldsymbol{+1}$ \textbf{SD} \\
\midrule

Trust formation
& Human Trust Propensity
& Safety Concern $\rightarrow$ Trust
& .060
& [.032, .088]
& $<.001$
& $-.199$
& $-.139$
& $-.079$ \\

Trust formation
& Objective Financial Literacy
& Source Knowledge $\rightarrow$ Trust
& .037
& [.013, .061]
& .041
& $.083$
& $.119$
& $.156$ \\

Reliance
& Objective Financial Literacy
& Trust $\rightarrow$ Reliance
& .039
& [.018, .060]
& .002
& $.562$
& $.601$
& $.640$ \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.97\textwidth}
\footnotesize
\textit{Note.}
Continuous moderators, appraisal variables, Trust, and Reliance were
standardized. The Trust-formation models included all appraisal
predictors, communication style, displayed source label, decision-context
characteristics, familiarity, and a participant random intercept.
The Reliance models additionally included Overall Quality, the four
appraisals, and Trust. Benjamini--Hochberg FDR correction was applied
within the 35 appraisal-to-Trust moderation tests and within the seven
Trust-to-Reliance moderation tests. Full moderation results are reported
in the Appendix.
\end{minipage}

\end{table*}

==> tables/21_trust_full_moderator.tex <==
\begin{table*}[t]
\sffamily
\centering
\small

\caption{
Complete screen of individual-difference moderation of the
appraisal-to-Trust pathway. Cells report standardized interaction
coefficients with Benjamini--Hochberg FDR-adjusted $p$-values in
parentheses.
}
\label{tab:moderator-screen}

\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.25}

\begin{tabular}{
    p{0.22\textwidth}
    c
    c
    c
    c
    c
}
\toprule
\textbf{Moderator}
& \textbf{Message}
& \textbf{Risk Ack.}
& \textbf{Safety}
& \textbf{Source Know.}
& \textbf{Quality} \\
\midrule

Human Trust Propensity
& $-.034$ (.117)
& $-.013$ (.553)
& $\mathbf{.060}$ ($\mathbf{<.001}$)
& $-.034$ (.117)
& $-.031$ (.155) \\

General AI Trust
& $-.015$ (.417)
& $.023$ (.279)
& $.041$ (.072)
& $.002$ (.941)
& $-.021$ (.292) \\

AI Literacy
& $.005$ (.876)
& $.029$ (.162)
& $.023$ (.292)
& $.009$ (.702)
& $-.002$ (.941) \\

Objective Financial Literacy
& $-.013$ (.417)
& $-.004$ (.906)
& $.026$ (.204)
& $\mathbf{.037}$ ($\mathbf{.041}$)
& $.022$ (.279) \\

Self-rated Financial Literacy
& $-.023$ (.292)
& $-.021$ (.292)
& $.013$ (.553)
& $.000$ (.995)
& $-.006$ (.839) \\

Risk Tolerance
& $-.021$ (.349)
& $-.006$ (.839)
& $.043$ (.072)
& $.000$ (.995)
& $-.019$ (.404) \\

AI Use for Finance
& $-.013$ (.553)
& $.010$ (.666)
& $.025$ (.279)
& $-.003$ (.941)
& $-.021$ (.292) \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.96\textwidth}
\footnotesize
\textit{Note.}
Each cell represents a separate pathway $\times$ moderator interaction
from a mixed-effects Trust model containing the full set of appraisal
and experimental covariates. Values in parentheses are
Benjamini--Hochberg FDR-adjusted $p$-values across all 35 interaction
tests. Boldface indicates $p_{\mathrm{FDR}}<.05$.
\end{minipage}

\end{table*}

==> tables/22_individualModerators_main.tex <==
\begin{table}[t]
\centering
\sffamily
\caption{Omnibus tests of individual-difference moderation of the
evaluation-to-Trust mechanism. Each likelihood-ratio test compares an
additive mixed-effects model with a model jointly adding the moderator's
interactions with Message Appraisal, Risk Acknowledgement, Safety Concern,
Source Knowledge, and Overall Quality.}
\label{tab:trust-moderator-omnibus}

\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lrrr}
\toprule
\textbf{Moderator}
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& 15.32 & 5 & \textbf{.021} \\

AI Literacy
& 8.45 & 5 & .186 \\

Human Trust Propensity
& 19.95 & 5 & \textbf{.005} \\

Objective Financial Literacy
& 26.45 & 5 & \textbf{$<$.001} \\

Self-rated Financial Literacy
& 6.51 & 5 & .260 \\

Risk Tolerance
& 10.28 & 5 & .118 \\

AI Use for Finance
& 7.38 & 5 & .226 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.97\linewidth}
\footnotesize
\textit{Note.} Benjamini--Hochberg FDR correction was applied across the
seven moderator-level omnibus tests. Significant omnibus tests were
followed by pathway-specific interaction tests.
\end{minipage}
\end{table}



\begin{table*}[t]
\centering
\sffamily
\caption{Localized individual-difference moderation and simple slopes for
significant pathways.}
\label{tab:individual-difference-simple-slopes}

% \setlength{\tabcolsep}{7pt}
% \renewcommand{\arraystretch}{1.18}

\resizebox{\columnwidth}{!}{\begin{tabular}{
    p{0.24\textwidth}
    p{0.23\textwidth}
    c
    c
    c
    c
}
\toprule
\textbf{Moderator}
& \textbf{Moderated pathway}
& $\boldsymbol{\beta_{\mathrm{int}}}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& \textbf{Moderator level}
& \textbf{Simple slope [95\% CI]} \\
\midrule

Objective Financial Literacy
& Source Knowledge $\rightarrow$ Trust
& .054
& \textbf{.017}
& $-1$ SD
& .074 [.020, .127] \\

&
&
&
&
Mean
& .127 [.080, .174] \\

&
&
&
&
$+1$ SD
& .181 [.117, .245] \\

\addlinespace[0.35em]

Human Trust Propensity
& Safety Concern $\rightarrow$ Trust
& .056
& \textbf{.002}
& $-1$ SD
& $-.193$ [$-.242$, $-.144$] \\

&
&
&
&
Mean
& $-.136$ [$-.171$, $-.102$] \\

&
&
&
&
$+1$ SD
& $-.080$ [$-.123$, $-.038$] \\

\addlinespace[0.35em]

Objective Financial Literacy
& Trust $\rightarrow$ Reliance
& .039
& \textbf{.002}
& $-1$ SD
& .562 [.509, .614] \\

&
&
&
&
Mean
& .601 [.551, .651] \\

&
&
&
&
$+1$ SD
& .640 [.585, .696] \\

\bottomrule
\end{tabular}}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.} Interaction coefficients are standardized regression
coefficients. For Trust formation, pathway-specific $p$-values were
Benjamini--Hochberg corrected across the five follow-up interactions
within each significant moderator block. For Trust-to-Reliance
moderation, FDR correction was applied across the seven moderator tests.
Simple slopes evaluate the focal association at one SD below the moderator
mean, at the mean, and one SD above the mean.
\end{minipage}
\end{table*}

==> tables/22_reliance_full_moderator.tex <==
\begin{table}[t]
\sffamily
\centering

\caption{
Moderation of the Trust--Reliance association by participant characteristics.
}
\label{tab:reliance-moderators}

\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lrr}
\toprule
\textbf{Moderator}
& $\boldsymbol{\beta_{\mathrm{int}}}$
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& $-.026$ & $.068$ \\

AI Literacy
& $.014$ & $.407$ \\

Human Trust Propensity
& $-.019$ & $.249$ \\

Objective Financial Literacy
& $\mathbf{.039}$
& $\mathbf{.002}$ \\

Self-rated Financial Literacy
& $.013$ & $.407$ \\

Risk Tolerance
& $-.003$ & $.794$ \\

AI Use for Finance
& $-.010$ & $.436$ \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.95\linewidth}
\footnotesize
\textit{Note.}
Coefficients correspond to Trust $\times$ moderator interactions predicting
Reliance in participant random-intercept mixed-effects models.
Benjamini--Hochberg FDR correction was applied across the seven interaction
tests. Boldface indicates $p_{\mathrm{FDR}}<.05$.
\end{minipage}

\end{table}

==> tables/23_individualmoderators.tex <==
\begin{table*}[t]
\centering
\sffamily
\caption{Participant-level associations with Trust before and after
accounting for advice evaluations.}
\label{tab:trust-moderator-main-effects}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.30\textwidth}
    cc
    cc
}
\toprule
&
\multicolumn{2}{c}{\textbf{Upstream model}}
&
\multicolumn{2}{c}{\textbf{Appraisal-adjusted model}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}

\textbf{Participant characteristic}
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& .202 & \textbf{$<$.001}
& .046 & .109 \\

AI Literacy
& .090 & .104
& $-.045$ & .109 \\

Human Trust Propensity
& .063 & .121
& .048 & .056 \\

Objective Financial Literacy
& .083 & .091
& $-.003$ & .977 \\

Self-rated Financial Literacy
& .016 & .692
& .005 & .977 \\

Risk Tolerance
& $-.077$ & .104
& .021 & .535 \\

AI Use for Finance
& $-.040$ & .427
& .001 & .977 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.} All seven participant characteristics were entered
simultaneously. The upstream model additionally controlled for
communication style, displayed label, decision context, and familiarity.
The appraisal-adjusted model additionally included Message Appraisal,
Risk Acknowledgement, Safety Concern, Source Knowledge, and Overall
Quality. FDR correction was applied across the seven participant-level
coefficients separately within each model.
\end{minipage}
\end{table*}


\begin{table*}[t]
\centering
\sffamily
\caption{Pathway-specific follow-up tests for participant characteristics
showing significant omnibus moderation of Trust formation.}
\label{tab:trust-moderator-followups}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.28\textwidth}
    p{0.30\textwidth}
    cc
}
\toprule
\textbf{Moderator}
& \textbf{Evaluation pathway}
& $\boldsymbol{\beta_{\mathrm{int}}}$
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

\multicolumn{4}{l}{\textit{General AI Trust}} \\

& Message Appraisal       & $-.003$ & .877 \\
& Risk Acknowledgement    & .032    & .140 \\
& Safety Concern          & .031    & .140 \\
& Source Knowledge        & .033    & .171 \\
& Overall Quality         & $-.044$ & .140 \\

\addlinespace[0.4em]
\multicolumn{4}{l}{\textit{Human Trust Propensity}} \\

& Message Appraisal       & .000    & .995 \\
& Risk Acknowledgement    & $-.002$ & .995 \\
& Safety Concern          & \textbf{.056} & \textbf{.002} \\
& Source Knowledge        & $-.024$ & .663 \\
& Overall Quality         & .008    & .995 \\

\addlinespace[0.4em]
\multicolumn{4}{l}{\textit{Objective Financial Literacy}} \\

& Message Appraisal       & $-.036$ & .055 \\
& Risk Acknowledgement    & $-.028$ & .076 \\
& Safety Concern          & .032    & .055 \\
& Source Knowledge        & \textbf{.054} & \textbf{.017} \\
& Overall Quality         & .028    & .213 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.} Each coefficient comes from the corresponding joint
five-interaction moderator model. Benjamini--Hochberg correction was
applied across the five pathway-specific follow-up tests within each
moderator block. Bold values indicate $p_{\mathrm{FDR}}<.05$.
\end{minipage}
\end{table*}


\begin{table*}[t]
\centering
\sffamily
\caption{Participant-level associations with intended Reliance across
successive adjustment stages.}
\label{tab:reliance-moderator-main-effects}

\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.27\textwidth}
    cc
    cc
    cc
}
\toprule
&
\multicolumn{2}{c}{\textbf{Upstream}}
&
\multicolumn{2}{c}{\textbf{Appraisals + Quality}}
&
\multicolumn{2}{c}{\textbf{Full mechanism}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}

\textbf{Participant characteristic}
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& .227 & \textbf{$<$.001}
& .080 & \textbf{.003}
& .053 & \textbf{.009} \\

AI Literacy
& .084 & .091
& $-.046$ & .122
& $-.018$ & .605 \\

Human Trust Propensity
& .042 & .267
& .029 & .242
& .001 & .993 \\

Objective Financial Literacy
& .076 & .084
& $-.005$ & .936
& $-.002$ & .993 \\

Self-rated Financial Literacy
& .011 & .779
& .002 & .941
& .000 & .993 \\

Risk Tolerance
& $-.082$ & .084
& .012 & .765
& .000 & .993 \\

AI Use for Finance
& $-.065$ & .186
& $-.024$ & .471
& $-.025$ & .397 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.} All models include communication style, displayed label,
decision-context characteristics, familiarity, and all seven participant
characteristics. The second model additionally includes Message Appraisal,
Risk Acknowledgment, Safety Concern, Source Knowledge, and Overall
Quality. The full-mechanism model additionally includes Trust. FDR
correction was applied across the seven participant characteristics
separately within each stage.
\end{minipage}
\end{table*}

\begin{table}[t]
\centering
\sffamily
\caption{Moderation of the association between Trust and intended
Reliance.}
\label{tab:trust-reliance-moderation}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lcc}
\toprule
\textbf{Moderator}
& $\boldsymbol{\beta_{\mathrm{int}}}$
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& $-.026$ & .068 \\

AI Literacy
& .014 & .407 \\

Human Trust Propensity
& $-.019$ & .249 \\

Objective Financial Literacy
& \textbf{.039} & \textbf{.002} \\

Self-rated Financial Literacy
& .013 & .407 \\

Risk Tolerance
& $-.003$ & .794 \\

AI Use for Finance
& $-.010$ & .436 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.} Coefficients represent Trust$\times$Moderator interaction
terms from mixed-effects models predicting Reliance while accounting for
Overall Quality, the four appraisal variables, communication style,
displayed label, decision context, and familiarity. FDR correction was
applied across the seven moderator tests.
\end{minipage}
\end{table}


\begin{table*}[t]
\centering
\sffamily
\caption{Omnibus tests of participant-characteristic moderation of
communication-style and displayed-label effects on Trust.}
\label{tab:style-label-moderation}

\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.28\textwidth}
    rcc
    rcc
}
\toprule
&
\multicolumn{3}{c}{\textbf{Communication Style}}
&
\multicolumn{3}{c}{\textbf{Displayed Label}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}

\textbf{Moderator}
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& 7.20 & 2 & .192
& 9.07 & 3 & .198 \\

AI Literacy
& 1.34 & 2 & .717
& 1.47 & 3 & .903 \\

Human Trust Propensity
& 0.63 & 2 & .852
& 0.57 & 3 & .903 \\

Objective Financial Literacy
& 0.13 & 2 & .936
& 1.80 & 3 & .903 \\

Self-rated Financial Literacy
& 1.97 & 2 & .654
& 3.22 & 3 & .903 \\

Risk Tolerance
& 4.30 & 2 & .271
& 2.96 & 3 & .903 \\

AI Use for Finance
& 4.71 & 2 & .271
& 0.62 & 3 & .903 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.} For communication style, each likelihood-ratio test
compares the additive Trust model with a model additionally containing
the two Style$\times$Moderator interactions; displayed label remains
additive. For displayed label, the comparison instead adds the three
Label$\times$Moderator interactions while communication style remains
additive. FDR correction was applied separately across the seven Style
tests and seven Label tests.
\end{minipage}
\end{table*}


==> tables/24_equations_ind_moderators.tex <==
\begin{table*}[t]
\centering
\sffamily
\small

\caption{Mixed-effects model specifications for participant-level
associations with advice appraisals, Trust, and Reliance.}
\label{tab:individual-main-models}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{
    p{0.29\textwidth}
    p{0.64\textwidth}
}
\toprule
\textbf{Model}
& \textbf{Specification} \\
\midrule

Initial appraisal
&
$A^{(k)}_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+u_i+\epsilon_{ij},
\quad
k\in\{\mathrm{Msg,Risk,Safety,Know}\}$
\\

\midrule

Trust: upstream
&
$T_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+u_i+\epsilon_{ij}$
\\

Trust: appraisal-adjusted
&
$T_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+\mathcal{A}_{ij}
+Q_{ij}
+u_i+\epsilon_{ij}$
\\

\midrule

Reliance: upstream
&
$R_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+u_i+\epsilon_{ij}$
\\

Reliance: appraisal + quality adjusted
&
$R_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+\mathcal{A}_{ij}
+Q_{ij}
+u_i+\epsilon_{ij}$
\\

Reliance: full mechanism adjusted
&
$R_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+\mathcal{A}_{ij}
+Q_{ij}
+T_{ij}
+u_i+\epsilon_{ij}$
\\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.}
$i$ indexes participants and $j$ repeated advice evaluations.
$\mathcal{C}$ contains communication style, displayed source label,
stakes, external uncertainty, verifiability, and scenario familiarity.
$\mathcal{A}$ contains Message Appraisal, Risk Acknowledgment,
Safety Concern, and Source Knowledge.
$A^{(k)}$ denotes one of these four appraisal outcomes.
$\mathcal{P}$ denotes the seven participant characteristics entered jointly.
$Q$, $T$, and $R$ denote Overall Quality, Trust, and Reliance,
respectively; $u_i$ denotes the participant random intercept.
\end{minipage}
\end{table*}


\begin{table*}[t]
\centering
\sffamily
\small

\caption{Mixed-effects model specifications for individual-difference
moderation analyses.}
\label{tab:individual-moderation-models}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.24}

\begin{tabular}{
    p{0.29\textwidth}
    p{0.64\textwidth}
}
\toprule
\textbf{Analysis}
& \textbf{Specification} \\
\midrule

Trust formation: additive
&
$T_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+M_i
+u_i+\epsilon_{ij}$
\\

Trust formation: moderator block
&
$T_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+M_i
+M_i\times(\mathcal{A}_{ij}+Q_{ij})
+u_i+\epsilon_{ij}$
\\

\midrule

Trust $\rightarrow$ Reliance moderation
&
$R_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+T_{ij}
+M_i
+(T_{ij}\times M_i)
+u_i+\epsilon_{ij}$
\\

\midrule

Style moderation of Trust
&
$T_{ij}
=
\mathcal{C}_{ij}
+M_i
+(\mathrm{Style}_{ij}\times M_i)
+u_i+\epsilon_{ij}$
\\

Label moderation of Trust
&
$T_{ij}
=
\mathcal{C}_{ij}
+M_i
+(\mathrm{Label}_{ij}\times M_i)
+u_i+\epsilon_{ij}$
\\

\midrule

Style moderation of appraisal
&
$A^{(k)}_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+(\mathrm{Style}_{ij}\times M_i)
+u_i+\epsilon_{ij}$
\\

Label moderation of appraisal
&
$A^{(k)}_{ij}
=
\mathcal{C}_{ij}
+\mathcal{P}_{i}
+(\mathrm{Label}_{ij}\times M_i)
+u_i+\epsilon_{ij}$
\\

\midrule

Simple slope
&
$\displaystyle
\mathrm{Slope}_{X\rightarrow Y}(M=m)
=
\beta_X + m\beta_{X\times M},
\qquad m\in\{-1,0,+1\}$
\\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.}
$M_i$ denotes the focal standardized participant-level moderator.
For Trust formation, the moderator block jointly adds interactions with
Message Appraisal, Risk Acknowledgment, Safety Concern, Source Knowledge,
and Overall Quality; the additive and moderator-block models were compared
using a 5-df likelihood-ratio test. Trust-to-Reliance moderation tests a
single $T\times M$ interaction. Style moderation adds the two
Style$\times M$ terms while displayed source label remains additive;
Label moderation analogously adds the three Label$\times M$ terms while
communication style remains additive. Targeted appraisal-moderation tests
used the same logic while retaining all seven participant characteristics
as additive predictors. For significant localized interactions, simple
slopes were evaluated at $m=-1$, $0$, and $+1$, corresponding to one
standard deviation below the moderator mean, the mean, and one standard
deviation above the mean.
\end{minipage}
\end{table*}

==> tables/25_decisioncontext_main.tex <==
\begin{table*}[t]
\centering
\sffamily

\caption{Omnibus tests of decision-context moderation of the Trust and
Reliance mechanisms.}
\label{tab:context-moderation}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.18}

\begin{tabular}{
    p{0.28\textwidth}
    rrr
    rrr
}
\toprule
&
\multicolumn{3}{c}{\textbf{Trust}}
&
\multicolumn{3}{c}{\textbf{Reliance}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}

\textbf{Decision-context dimension}
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

Stakes
& 11.52 & 5 & .104
& 5.22 & 6 & .737 \\

External Uncertainty
& 10.23 & 5 & .104
& 13.17 & 6 & .121 \\

Verifiability
& 5.94 & 5 & .312
& 3.55 & 6 & .737 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.}
For Trust, each likelihood-ratio test compared the additive mixed-effects
model with a model jointly adding interactions between the focal
decision-context dimension and Message Appraisal, Risk Acknowledgment,
Safety Concern, Source Knowledge, and Overall Quality. For Reliance,
Trust was additionally included as a sixth moderated pathway.
All models retained communication style, displayed source label, all
three decision-context main effects, scenario familiarity, and a
participant random intercept. Models were fitted using maximum likelihood
for fixed-effect comparisons. Benjamini--Hochberg FDR correction was
applied across the three context tests separately for Trust and Reliance.
\end{minipage}
\end{table*}

==> tables/26_decisionContext_equations.tex <==
\begin{table*}[t]
\centering
\sffamily
\small

\caption{Model specifications for decision-context moderation analyses.}
\label{tab:context-model-specifications}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{
    p{0.25\textwidth}
    p{0.67\textwidth}
}
\toprule
\textbf{Model}
& \textbf{Specification} \\
\midrule

Trust: additive
&
$T_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+u_i+\epsilon_{ij}$
\\

Trust: context moderation
&
$T_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+D_{ij}\times(\mathcal{A}_{ij}+Q_{ij})
+u_i+\epsilon_{ij}$
\\

\midrule

Reliance: additive
&
$R_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+T_{ij}
+u_i+\epsilon_{ij}$
\\

Reliance: context moderation
&
$R_{ij}
=
\mathcal{C}_{ij}
+\mathcal{A}_{ij}
+Q_{ij}
+T_{ij}
+D_{ij}\times(\mathcal{A}_{ij}+Q_{ij}+T_{ij})
+u_i+\epsilon_{ij}$
\\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.96\linewidth}
\footnotesize
\textit{Note.}
$i$ indexes participants and $j$ repeated advice evaluations.
$D_{ij}$ denotes the focal decision-context dimension
(Stakes, External Uncertainty, or Verifiability).
$\mathcal{A}$ contains Message Appraisal, Risk Acknowledgment,
Safety Concern, and Source Knowledge; $Q$, $T$, and $R$ denote Overall
Quality, Trust, and Reliance, respectively.
$\mathcal{C}$ contains communication style, displayed source label,
all three decision-context main effects, and scenario familiarity.
$u_i$ denotes the participant random intercept.
For each decision-context dimension, the additive and interaction models
were compared using maximum likelihood. The Trust comparison adds five
interaction terms ($df=5$); the Reliance comparison adds six
($df=6$).
\end{minipage}
\end{table*}


==> tables/27_robustness_1.tex <==
\begin{table}[t]
\sffamily
\centering
\small

\caption{
Within- and between-participant decomposition predicting Overall Quality.
}
\label{tab:wb-quality}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Within participant}}
& \multicolumn{2}{c}{\textbf{Between participant}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}

\textbf{Predictor}
& $\boldsymbol{\beta_W}$
& $\boldsymbol{p_W}$
& $\boldsymbol{\beta_B}$
& $\boldsymbol{p_B}$ \\
\midrule

Message Appraisal
& .329 & $<.001$
& .289 & $<.001$ \\

Risk Acknowledgement
& .073 & .001
& .069 & .046 \\

Safety Concern
& -.106 & $<.001$
& -.072 & .018 \\

Source Knowledge
& .444 & $<.001$
& .602 & $<.001$ \\

Familiarity
& .019 & .428
& .053 & .066 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.94\linewidth}
\footnotesize
\textit{Note.}
Within-participant coefficients capture deviations from each
participant's own mean; between-participant coefficients capture
differences in participants' average evaluations. Models additionally
included advice style, displayed source label, decision-context
characteristics, and a participant random intercept. Continuous
evaluation variables were standardized.
\end{minipage}

\end{table}


\begin{table}[t]
\sffamily
\centering
\small

\caption{
Within- and between-participant decomposition predicting Trust.
}
\label{tab:wb-trust}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Within participant}}
& \multicolumn{2}{c}{\textbf{Between participant}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}

\textbf{Predictor}
& $\boldsymbol{\beta_W}$
& $\boldsymbol{p_W}$
& $\boldsymbol{\beta_B}$
& $\boldsymbol{p_B}$ \\
\midrule

Message Appraisal
& .147 & $<.001$
& .091 & .040 \\

Risk Acknowledgement
& .048 & .018
& -.035 & .253 \\

Safety Concern
& -.159 & $<.001$
& -.073 & .007 \\

Source Knowledge
& .108 & $<.001$
& .093 & .064 \\

Overall Quality
& .573 & $<.001$
& .701 & $<.001$ \\

Familiarity
& .037 & .091
& .042 & .103 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.94\linewidth}
\footnotesize
\textit{Note.}
Within-participant coefficients capture deviations from each
participant's own mean; between-participant coefficients capture
differences in participants' average evaluations. Models additionally
included advice style, displayed source label, decision-context
characteristics, and a participant random intercept. Continuous
evaluation variables were standardized.
\end{minipage}

\end{table}



\begin{table}[t]
\sffamily
\centering
\small

\caption{
Within- and between-participant decomposition predicting Reliance.
}
\label{tab:wb-reliance}

\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.20}

\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Within participant}}
& \multicolumn{2}{c}{\textbf{Between participant}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}

\textbf{Predictor}
& $\boldsymbol{\beta_W}$
& $\boldsymbol{p_W}$
& $\boldsymbol{\beta_B}$
& $\boldsymbol{p_B}$ \\
\midrule

Message Appraisal
& .113 & $<.001$
& .018 & .571 \\

Risk Acknowledgement
& -.002 & .895
& -.022 & .307 \\

Safety Concern
& -.087 & $<.001$
& -.020 & .302 \\

Source Knowledge
& .035 & .157
& .073 & .038 \\

Overall Quality
& .221 & $<.001$
& .175 & $<.001$ \\

Trust
& .533 & $<.001$
& .682 & $<.001$ \\

Familiarity
& .089 & $<.001$
& .012 & .500 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.94\linewidth}
\footnotesize
\textit{Note.}
Within-participant coefficients capture deviations from each
participant's own mean; between-participant coefficients capture
differences in participants' average evaluations. Models additionally
included advice style, displayed source label, decision-context
characteristics, and a participant random intercept. Continuous
evaluation variables were standardized.
\end{minipage}

\end{table}



==> tables/28_robustness_2.tex <==
\begin{table*}[t]
\sffamily
\centering
\small

\caption{
Generalized estimating equation (GEE) replication of the core
evaluation-pathway models. Models used a Gaussian family with an
exchangeable working correlation to account for repeated evaluations
within participants. Coefficients are standardized; $p$-values are
reported below each coefficient.
}
\label{tab:gee-robustness}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.30}

\begin{tabular}{
    p{0.25\textwidth}
    c
    c
    c
}
\toprule
\textbf{Predictor}
& \textbf{Overall Quality}
& \textbf{Trust}
& \textbf{Reliance} \\
\midrule

Message Appraisal
& $\mathbf{.325}$ \newline $(p<.001)$
& $\mathbf{.132}$ \newline $(p<.001)$
& $\mathbf{.078}$ \newline $(p=.002)$ \\

Risk Acknowledgement
& $\mathbf{.075}$ \newline $(p=.001)$
& $.024$ \newline $(p=.148)$
& $-.016$ \newline $(p=.274)$ \\

Safety Concern
& $\mathbf{-.088}$ \newline $(p<.001)$
& $\mathbf{-.125}$ \newline $(p<.001)$
& $\mathbf{-.049}$ \newline $(p=.002)$ \\

Source Knowledge
& $\mathbf{.489}$ \newline $(p<.001)$
& $\mathbf{.109}$ \newline $(p<.001)$
& $.048$ \newline $(p=.084)$ \\

Overall Quality
& ---
& $\mathbf{.608}$ \newline $(p<.001)$
& $\mathbf{.206}$ \newline $(p<.001)$ \\

Trust
& ---
& ---
& $\mathbf{.595}$ \newline $(p<.001)$ \\

\bottomrule
\end{tabular}

\vspace{0.4em}

\begin{minipage}{0.96\textwidth}
\footnotesize
\textit{Note.}
All models additionally controlled for communication style, displayed
source label, stakes, external uncertainty, verifiability, and
familiarity. Boldface indicates $p<.05$. GEE estimates closely
reproduced the participant random-intercept mixed-effects models used in
the primary analysis. The only change in inferential significance was
the small direct Source Knowledge--Reliance association, which remained
similar in magnitude but was not statistically distinguishable from zero
under GEE.
\end{minipage}

\end{table*}

==> tables/29_robustness_3.tex <==
\begin{table*}[t]
\sffamily
\centering
\small

\caption{
Robustness of the evaluation pathway to scenario fixed effects.
The primary models represent decision context using stakes, external
uncertainty, and verifiability; the robustness models replace these
terms with fixed effects for each of the eight financial scenarios.
Coefficients are standardized.
}
\label{tab:scenario-fe-robustness}

\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.25}

\begin{tabular}{
    l
    r
    r
}
\toprule
\textbf{Pathway}
& \textbf{Primary model}
& \textbf{Scenario FE} \\
\midrule

\multicolumn{3}{l}{\textit{Panel A: Overall Quality}} \\[0.15em]

Message Appraisal $\rightarrow$ Overall Quality
& .325*** & .320*** \\

Risk Acknowledgment $\rightarrow$ Overall Quality
& .075*** & .075*** \\

Safety Concern $\rightarrow$ Overall Quality
& $-.088$*** & $-.088$*** \\

Source Knowledge $\rightarrow$ Overall Quality
& .489*** & .491*** \\

\addlinespace
\multicolumn{3}{l}{\textit{Panel B: Trust}} \\[0.15em]

Message Appraisal $\rightarrow$ Trust
& .132*** & .130*** \\

Risk Acknowledgment $\rightarrow$ Trust
& .024 & .025 \\

Safety Concern $\rightarrow$ Trust
& $-.125$*** & $-.125$*** \\

Source Knowledge $\rightarrow$ Trust
& .109*** & .111*** \\

Overall Quality $\rightarrow$ Trust
& .607*** & .603*** \\

\addlinespace
\multicolumn{3}{l}{\textit{Panel C: Reliance}} \\[0.15em]

Message Appraisal $\rightarrow$ Reliance
& .079*** & .080*** \\

Risk Acknowledgment $\rightarrow$ Reliance
& $-.015$ & $-.012$ \\

Safety Concern $\rightarrow$ Reliance
& $-.050$*** & $-.050$*** \\

Source Knowledge $\rightarrow$ Reliance
& .047* & .046* \\

Overall Quality $\rightarrow$ Reliance
& .206*** & .206*** \\

Trust $\rightarrow$ Reliance
& .594*** & .593*** \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.95\textwidth}
\footnotesize
\textit{Note.}
Primary models include stakes, external uncertainty, and verifiability
as decision-context covariates. Scenario-FE models instead include a
fixed effect for each financial scenario, absorbing stable
scenario-specific heterogeneity. All models retain communication style,
displayed source attribution, familiarity, and a participant random
intercept. $^{*}p<.05$, $^{**}p<.01$, $^{***}p<.001$.
\end{minipage}

\end{table*}

==> tables/2_decision_context_definitions.tex <==
% Table: Scenario-level vignette dimensions
\begin{table}[t]
\centering
\sffamily

\caption{Scenario-level dimensions in the 2 $\times$ 2 $\times$ 2 vignette design.}
\label{tab:scenario_dimensions}
% \small
\begin{tabular}{p{0.10\linewidth} p{0.30\linewidth} p{0.23\linewidth} p{0.23\linewidth}}
\textbf{Dimension} & \textbf{Definition} & \textbf{Low level} & \textbf{High level} \\
\toprule
% \midrule
Stakes &
Magnitude and long-term financial consequences of the decision. &
Smaller or more reversible decisions, such as travel insurance or short-term spending choices. &
Substantial or difficult-to-reverse decisions, such as graduate school, debt repayment, or concentrated investment risk. \\

External uncertainty &
Whether outcomes depend on unpredictable future conditions. &
Outcomes are relatively stable or calculable, such as fixed interest rates or known rent differences. &
Outcomes depend on external events, such as market volatility, weather disruptions, or future job-market conditions. \\

Verifiability &
Whether advice quality can be evaluated against established financial principles. &
Preference-sensitive decisions with no single dominant rule, such as housing lifestyle trade-offs or graduate-school ROI. &
Decisions with broad expert consensus, such as paying high-interest debt or diversifying concentrated assets. \\
\bottomrule
\end{tabular}
\end{table}

==> tables/30_robustness_4.tex <==
\begin{table*}[t]
\centering
\sffamily
\small

\caption{
Item-level sensitivity analysis for the evaluation pathway.
The Message Appraisal and Safety Concern composites were replaced by
their constituent items while retaining the remaining predictors and
controls from the primary models.
}
\label{tab:item-level-sensitivity}

\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.35}

\begin{tabular}{
    p{0.28\textwidth}
    c
    c
    c
}
\toprule
\textbf{Predictor}
& \textbf{Overall Quality}
& \textbf{Trust}
& \textbf{Reliance} \\
\midrule

\rowcolor{blue!5}
Readability
& $.045$ \newline {\scriptsize $(p=.096)$}
& $\mathbf{.057}$ \newline {\scriptsize $(p=.020)$}
& $.035$ \newline {\scriptsize $(p=.088)$} \\

Reasoning Clarity
& $\mathbf{.109}$ \newline {\scriptsize $(p<.001)$}
& $.026$ \newline {\scriptsize $(p=.341)$}
& $.041$ \newline {\scriptsize $(p=.079)$} \\

\rowcolor{blue!5}
Situational Fit
& $\mathbf{.226}$ \newline {\scriptsize $(p<.001)$}
& $\mathbf{.073}$ \newline {\scriptsize $(p=.004)$}
& $.009$ \newline {\scriptsize $(p=.673)$} \\

Risk Acknowledgement
& $\mathbf{.074}$ \newline {\scriptsize $(p<.001)$}
& $.028$ \newline {\scriptsize $(p=.104)$}
& $-.015$ \newline {\scriptsize $(p=.275)$} \\

\rowcolor{blue!5}
Financial Harm Risk
& $\mathbf{-.085}$ \newline {\scriptsize $(p<.001)$}
& $\mathbf{-.113}$ \newline {\scriptsize $(p<.001)$}
& $\mathbf{-.034}$ \newline {\scriptsize $(p=.030)$} \\

Misleadingness
& $-.013$ \newline {\scriptsize $(p=.543)$}
& $-.031$ \newline {\scriptsize $(p=.098)$}
& $-.023$ \newline {\scriptsize $(p=.128)$} \\

\rowcolor{blue!5}
Source Knowledge
& $\mathbf{.465}$ \newline {\scriptsize $(p<.001)$}
& $\mathbf{.108}$ \newline {\scriptsize $(p<.001)$}
& $\mathbf{.048}$ \newline {\scriptsize $(p=.020)$} \\

Overall Quality
& --- 
& $\mathbf{.598}$ \newline {\scriptsize $(p<.001)$}
& $\mathbf{.208}$ \newline {\scriptsize $(p<.001)$} \\

\rowcolor{blue!5}
Trust
& ---
& ---
& $\mathbf{.594}$ \newline {\scriptsize $(p<.001)$} \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.95\textwidth}
\footnotesize
\textit{Note.}
Coefficients are standardized fixed-effect estimates from participant
random-intercept mixed-effects models. Models additionally controlled
for advice style, displayed source label, stakes, external uncertainty,
verifiability, and familiarity. Boldface indicates $p<.05$.
The constituent items are entered simultaneously; therefore, individual
coefficients represent each item's unique association after accounting
for the other correlated items. Joint tests of the corresponding item
blocks are reported in Table~\ref{tab:item-block-wald}.
\end{minipage}

\end{table*}

\begin{table}[t]
\centering
\sffamily
\small

\caption{
Joint Wald tests of constituent Message Appraisal and Safety Concern
items in the item-level sensitivity models.
}
\label{tab:item-block-wald}

\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.30}

\begin{tabular}{
    l
    c
    c
}
\toprule
\textbf{Outcome}
& \textbf{Message-item block}
& \textbf{Safety-item block} \\
\midrule

\rowcolor{blue!5}
Overall Quality
& $\chi^2(3)=211.04$ \newline {\scriptsize $(p<.001)$}
& $\chi^2(2)=23.70$ \newline {\scriptsize $(p<.001)$} \\

Trust
& $\chi^2(3)=35.79$ \newline {\scriptsize $(p<.001)$}
& $\chi^2(2)=56.55$ \newline {\scriptsize $(p<.001)$} \\

\rowcolor{blue!5}
Reliance
& $\chi^2(3)=16.67$ \newline {\scriptsize $(p<.001)$}
& $\chi^2(2)=12.45$ \newline {\scriptsize $(p=.002)$} \\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.94\linewidth}
\footnotesize
\textit{Note.}
The Message-item block jointly tests
$H_0:\beta_{\mathrm{Readability}}
=\beta_{\mathrm{Reasoning}}
=\beta_{\mathrm{Fit}}=0$.
The Safety-item block jointly tests
$H_0:\beta_{\mathrm{HarmRisk}}
=\beta_{\mathrm{Misleadingness}}=0$.
\end{minipage}

\end{table}

==> tables/32_ind_moderators_vs_appraisals_full.tex <==
\begin{table*}[t]
\centering
\sffamily
\small

\caption{Associations between participant characteristics and initial
advice appraisals.}
\label{tab:individual-appraisal-full}

\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.27\textwidth}
    cc
    cc
    cc
    cc
}
\toprule
&
\multicolumn{2}{c}{\textbf{Message Appraisal}}
&
\multicolumn{2}{c}{\textbf{Risk Acknowledgement}}
&
\multicolumn{2}{c}{\textbf{Safety Concern}}
&
\multicolumn{2}{c}{\textbf{Source Knowledge}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}

\textbf{Participant characteristic}
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\beta}$
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

General AI Trust
& .080 & .199
& .065 & .267
& $-.075$ & .377
& \textbf{.168} & \textbf{.001} \\

AI Literacy
& \textbf{.189} & \textbf{$<$.001}
& .125 & .065
& $-.007$ & .891
& \textbf{.178} & \textbf{$<$.001} \\

Human Trust Propensity
& $-.012$ & .836
& $-.074$ & .104
& .049 & .440
& $-.007$ & .853 \\

Objective Financial Literacy
& .058 & .213
& .087 & .104
& $-.081$ & .216
& \textbf{.086} & \textbf{.038} \\

Self-rated Financial Literacy
& .009 & .836
& .014 & .871
& .020 & .785
& .035 & .469 \\

Risk Tolerance
& $-.084$ & .141
& $-.086$ & .104
& \textbf{.145} & \textbf{.015}
& \textbf{$-.117$} & \textbf{.011} \\

AI Use for Finance
& $-.065$ & .213
& $-.005$ & .913
& .040 & .628
& $-.061$ & .249 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.97\linewidth}
\footnotesize
\textit{Note.}
All seven participant characteristics were entered simultaneously in each
appraisal model. Models additionally controlled for communication style,
displayed source label, stakes, external uncertainty, verifiability, and
scenario familiarity, with participant random intercepts.
Benjamini--Hochberg correction was applied across the seven
participant-characteristic tests separately within each appraisal.
Bold values indicate $p_{\mathrm{FDR}}<.05$.
\end{minipage}
\end{table*}


\begin{table*}[t]
\centering
\sffamily
\small

\caption{Targeted exploratory tests of whether participant-characteristic
associations with initial appraisals varied by communication style or
displayed source label.}
\label{tab:appraisal-style-label-mod}

\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{
    p{0.38\textwidth}
    rcc
    rcc
}
\toprule
&
\multicolumn{3}{c}{\textbf{Communication Style}}
&
\multicolumn{3}{c}{\textbf{Displayed Label}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}

\textbf{Focal relationship}
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$
& $\boldsymbol{\chi^2}$
& \textbf{df}
& $\boldsymbol{p_{\mathrm{FDR}}}$ \\
\midrule

AI Literacy $\rightarrow$ Message Appraisal
& 7.68 & 2 & .065
& 1.98 & 3 & .591 \\

AI Literacy $\rightarrow$ Source Knowledge
& 2.90 & 2 & .352
& 3.53 & 3 & .573 \\

General AI Trust $\rightarrow$ Source Knowledge
& 4.44 & 2 & .217
& 3.06 & 3 & .573 \\

Objective Financial Literacy $\rightarrow$ Source Knowledge
& 9.32 & 2 & .057
& 6.69 & 3 & .496 \\

Risk Tolerance $\rightarrow$ Safety Concern
& 0.95 & 2 & .621
& 1.91 & 3 & .591 \\

Risk Tolerance $\rightarrow$ Source Knowledge
& 1.03 & 2 & .621
& 3.82 & 3 & .573 \\

\bottomrule
\end{tabular}

\vspace{0.35em}
\begin{minipage}{0.97\linewidth}
\footnotesize
\textit{Note.}
Follow-up analyses were restricted to participant-characteristic/appraisal
associations that survived FDR correction in the preceding analysis.
For communication style, each likelihood-ratio test compared the additive
appraisal model with a model additionally containing the two
Style$\times$Characteristic interactions while displayed label remained
additive. Label moderation analogously added the three
Label$\times$Characteristic interactions while communication style
remained additive. Benjamini--Hochberg correction was applied separately
across the six Style and six Label omnibus tests. No interaction block
survived correction.
\end{minipage}
\end{table*}

==> tables/33_validation_main.tex <==
\begin{table*}[t]
\centering
\sffamily
\footnotesize
\caption{Selected linguistic profiles of the constructed stimuli and the external reference corpus. Values are means. Full results for all linguistic measures are reported in Appendix~\ref{app:stimulus_validation_details}.}
\label{tab:validation_profiles}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrrrrrr}
& \multicolumn{2}{c}{\textbf{AI}} & \multicolumn{2}{c}{\textbf{Expert}} & \multicolumn{2}{c}{\textbf{Online Community}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
\textbf{Measure} & \textbf{Constructed} & \textbf{Reference} & \textbf{Constructed} & \textbf{Reference} & \textbf{Constructed} & \textbf{Reference} \\
\toprule
% \midrule
Categorical--Dynamic Index & 27.36 & 27.31 & 21.30 & 22.92 & 12.03 & 12.05 \\
Formality & .824 & .530 & .801 & .733 & .521 & .572 \\
Coleman--Liau grade level & 13.67 & 12.04 & 13.39 & 11.45 & 7.74 & 7.11 \\
% Mean word length & 5.34 & 4.96 & 5.25 & 4.93 & 4.41 & 4.27 \\
First-person singular / 100 words & 0.00 & 0.14 & 0.62 & 0.59 & 3.66 & 1.97 \\
Contractions / 100 words & 0.00 & 1.15 & 1.59 & 1.43 & 3.58 & 2.55 \\
\bottomrule
\end{tabular}

\vspace{2pt}
\footnotesize\emph{Note.} Constructed values summarize eight stimuli per communication style; reference values summarize 24 topic-matched texts per source category. Higher CDI values indicate more categorical/analytical language, whereas lower values indicate more dynamic/interpersonal language. Higher formality scores indicate a greater probability of formal language. Coleman--Liau values represent approximate grade level rather than ``ease of reading.'' The appendix reports the complete feature set, including dimensions that did not show the same source ordering.
\end{table*}


==> tables/35_ranking_main.tex <==
\begin{table}[t]
\caption{First-ranked advice style in the comparative ranking task, overall and by displayed source-attribution condition. Percentages are calculated within each row.}
\label{tab:task2_rankings}
\centering
\small
\begin{tabular}{lrrrr}
\toprule
Condition & $N$ & AI & Expert & OC \\
\midrule
Overall     & 285 & 67 (23.5\%) & \textbf{135 (47.4\%)} & 83 (29.1\%) \\
Labeled     & 100 & 22 (22.0\%) & \textbf{53 (53.0\%)}  & 25 (25.0\%) \\
Unlabeled   & 92  & 19 (20.7\%) & \textbf{44 (47.8\%)}  & 29 (31.5\%) \\
Mislabeled  & 93  & 26 (28.0\%) & \textbf{38 (40.9\%)}  & 29 (31.2\%) \\
\bottomrule
\end{tabular}
\end{table}

==> tables/3_scenario_operationalization.tex <==
\begin{table*}[t]
\sffamily
\centering
\small

\caption{Operationalization of the decision-context taxonomy across the eight financial scenarios.}
\label{tab:scenario_taxonomy}

\begin{tabular}{
    p{0.20\textwidth}
    p{0.24\textwidth}
    p{0.25\textwidth}
    p{0.25\textwidth}
}
\toprule
\textbf{Scenario}
& \textbf{Stakes}
& \textbf{External uncertainty}
& \textbf{Verifiability} \\
\midrule

\textbf{1. Renting: Shared vs.\ Private}
&
\textbf{Low.}
Approximately \$1,000/month difference; primarily a lifestyle and savings trade-off; relatively reversible.
&
\textbf{Low.}
Costs are largely determined by known rent and income rather than unpredictable external conditions.
&
\textbf{Low.}
No dominant financial rule; decision depends substantially on preferences for privacy, independence, and savings.
\\[0.5em]

\textbf{2. Credit Card vs.\ New Laptop}
&
\textbf{Low.}
An \$800--\$1,000 short-term decision with limited effect on the individual's long-term financial trajectory.
&
\textbf{Low.}
The 22\% APR is fixed and the financial consequences of carrying the balance are readily calculable.
&
\textbf{High.}
A well-established principle favors paying high-interest revolving debt before making a discretionary purchase.
\\[0.5em]

\textbf{3. Travel Insurance}
&
\textbf{Low.}
The \$80 premium and \$1,200 trip cost are small relative to income and unlikely to materially affect long-term finances.
&
\textbf{High.}
Outcomes depend on uncertain events such as weather disruptions, cancellations, medical issues, or lost baggage.
&
\textbf{Low.}
No universally dominant choice; purchasing insurance depends on risk tolerance, preferences, and ability to absorb the loss.
\\[0.5em]

\textbf{4. Emergency Fund vs.\ Investing Bonus}
&
\textbf{Low.}
The \$2,000 allocation decision has limited long-term consequences and does not substantially alter the individual's financial position.
&
\textbf{High.}
The value of emergency savings depends on unpredictable expenses or events such as medical bills, repairs, or employment gaps.
&
\textbf{High.}
Established financial guidance generally recommends maintaining an adequate emergency reserve before prioritizing additional investment.
\\[0.5em]

\textbf{5. Graduate School vs.\ Continuing Work}
&
\textbf{High.}
The decision involves \$120,000 in tuition plus two years of forgone income and potentially substantial long-term career consequences.
&
\textbf{Low.}
The scenario assumes a stable near-term job market and predictable earnings, limiting dependence on external economic volatility.
&
\textbf{Low.}
There is no dominant financial rule; the decision depends on program quality, career goals, expected returns, and personal preferences.
\\[0.5em]

\textbf{6. High-Interest Debt Repayment and Budgeting}
&
\textbf{High.}
The scenario involves \$40,000 in student debt at approximately 10\% interest, with substantial implications for long-term financial well-being.
&
\textbf{Low.}
The loan rate is fixed and repayment consequences are largely deterministic.
&
\textbf{High.}
Established financial principles favor capturing the employer retirement match while prioritizing repayment of high-interest debt.
\\[0.5em]

\textbf{7. Long-Term Investment Planning}
&
\textbf{High.}
The allocation decision concerns long-term retirement savings and wealth accumulation over approximately 30 years.
&
\textbf{High.}
Future returns depend on market volatility and broader macroeconomic conditions that cannot be predicted with certainty.
&
\textbf{Low.}
No single allocation is optimal for all investors; the appropriate strategy depends on risk tolerance, horizon, and behavioral preferences.
\\[0.5em]

\textbf{8. Concentrated Stock Position Risk}
&
\textbf{High.}
Approximately 75\% of a \$240,000 portfolio is concentrated in employer stock, creating substantial exposure of personal wealth.
&
\textbf{High.}
Future outcomes depend on company performance, sector conditions, and broader market volatility.
&
\textbf{High.}
Diversification and reduction of excessive single-stock concentration are well-established portfolio-management principles.
\\

\bottomrule
\end{tabular}

\vspace{0.4em}
\begin{minipage}{0.96\textwidth}
\footnotesize
\textit{Note.}
Stakes captures the magnitude and long-term financial consequences of the decision; external uncertainty captures the extent to which outcomes depend on unpredictable future conditions; and verifiability captures whether advice quality can be evaluated against an established financial principle.
\end{minipage}

\end{table*}

==> tables/4_advicestyleOperationalization.tex <==
% Table: Operationalization of source-specific communication styles
\begin{table*}[t]
\centering
\caption{Operationalization of source-specific communication styles and
corresponding linguistic validation measures.}
\label{tab:advice_style_operationalization}

\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.18}

\begin{tabularx}{\textwidth}{
    >{\raggedright\arraybackslash}p{0.09\textwidth}
    >{\raggedright\arraybackslash}X
    >{\raggedright\arraybackslash}X
    >{\raggedright\arraybackslash}X
    >{\raggedright\arraybackslash}p{0.17\textwidth}
}
\toprule
\textbf{Feature}
& \textbf{AI advice}
& \textbf{Expert advice}
& \textbf{OC advice}
& \textbf{Validation measures} \\
\midrule

\textbf{Voice}
& Impersonal; no first-person identity
& Mild first-person professional authority
& First-person peer perspective
& First-person singular language \\

\textbf{Tone}
& Neutral and analytical
& Professional and measured
& Informal and conversational
& Formality; contractions \\

\textbf{Reasoning}
& Explicit analysis and conditional if--then reasoning
& Structured, principle-based reasoning oriented toward long-term planning
& Experiential reasoning supported by practical heuristics
& CDI; conditional markers; modal language \\

\textbf{Framing}
& Balances available options and evaluates financial risk exposure
& Connects the decision to financial foundations and broader goals
& Uses lived experience, subjective judgment, and relatable consequences
& CDI; first-person language \\

\textbf{Structure}
& Situation and trade-off; analysis; conditional recommendation
& Quantified framing; trade-off explanation; actionable principle
& Anecdote or position; experiential lesson; direct recommendation
& Words per sentence; Coleman--Liau grade level; lexical repetition \\

\textbf{Constrained features}
& Personal anecdotes, emotional validation, and unsupported personal assumptions
& Personal anecdotes, slang, and emotional storytelling
& Formal advisory authority and technical optimization language
& First-person language; contractions; formality \\

\bottomrule
\end{tabularx}

\vspace{3pt}

\begin{minipage}{\textwidth}
\footnotesize
\textit{Note.}
We define \textit{advice style} as a controlled bundle of message-level
features involving voice, tone, reasoning presentation, framing, and
discourse structure. Style was varied separately from a common substantive
decision backbone: within each scenario, vignette-relevant financial facts,
core financial principles, recommendation direction, and core rationale were
standardized across versions. Source-characteristic supporting rhetoric was
allowed to vary; in particular, OC responses could use experiential examples
or anecdotal evidence as part of their intended communication style.

The validation measures capture observable linguistic correlates of these
design dimensions rather than one-to-one operationalizations of each
construct. The complete linguistic battery additionally included response
length, mean word length, second-person language, hedging, and other lexical
markers; full definitions and results are reported in
Appendix~\ref{app:stimulus_validation_details}. Because some distinctions,
such as professional authority and experiential framing, operate at a broader
discourse level, linguistic analyses were complemented by independent human
ratings and blind source-style classification.

The three versions were constructed using source-specific drafting and
prompting instructions and manually reviewed for consistency with the common
decision backbone and approximate length. The constrained features represent
experimental design choices rather than claims that real-world sources never
exhibit these characteristics. The resulting stimuli should therefore be
understood as controlled source-associated communication profiles rather than
literal reproductions of all communication from each source category. The
participant-facing labels were ``AI Financial Assistant,'' ``Certified
Financial Planner,'' and ``Online Community Forum.''
\end{minipage}

\end{table*}

==> tables/5_evaluationItems.tex <==

% Table: Advice-evaluation measurement items
\begin{table*}[t]
\centering
\caption{Measurement items used to evaluate financial advice.}
\label{tab:measurement_items}
\renewcommand{\arraystretch}{1.18}
\setlength{\tabcolsep}{6pt}

\begin{tabularx}{\textwidth}{
    >{\centering\arraybackslash}p{0.05\textwidth}
    >{\raggedright\arraybackslash}X
    >{\raggedright\arraybackslash}p{0.25\textwidth}
}
\toprule
\textbf{No.} & \textbf{Measurement Item (7-point Likert scale)} & \textbf{Dimension} \\
\midrule

\multicolumn{3}{l}{\textit{\textbf{Presentation and Comprehension}}} \\
\addlinespace[2pt]
1 & The advice is easy to read and follow.
  & Readability \\

2 & The advice provides clear reasoning for its recommendation.
  & Reasoning clarity \\

3 & The advice fits well with X's situation.
  & Situational fit \\

\addlinespace[4pt]
\multicolumn{3}{l}{\textit{\textbf{Risk and Safety Perception}}} \\
\addlinespace[2pt]
4 & The advice acknowledges potential risks and uncertainties.
  & Risk acknowledgment \\

5 & Following this advice could put X at financial risk.
  & Financial harm risk$\dagger$ \\

6 & Someone with limited financial knowledge could misunderstand this advice.
  & Misleadingness$\dagger$ \\

\addlinespace[4pt]
\multicolumn{3}{l}{\textit{\textbf{Source Authority and Behavioral Intentions}}} \\
\addlinespace[2pt]
7 & The source of this advice appears knowledgeable about financial decisions.
  & Perceived source knowledge \\

8 & Overall, this is high-quality financial advice for X.
  & Perceived overall quality \\

9 & I would trust this advice if I were in X's situation.
  & Trust intention \\

10 & If I were in X's situation, I would feel comfortable following this advice.
  & Reliance intention \\

\bottomrule
\end{tabularx}

\vspace{3pt}
\begin{minipage}{\textwidth}
\footnotesize
\textit{Note.} X denotes the protagonist named in each financial scenario.
Items marked with dagger ($\dagger$) are negatively valenced: higher ratings indicate
greater perceived financial harm or misleadingness.
\end{minipage}
\end{table*}

==> tables/6_efa.tex <==
\begin{table}[t]
\sffamily
\footnotesize
\centering
\caption{Exploratory factor analysis and parallel analysis of the ten advice-evaluation items.
EFA used MINRES extraction with oblimin rotation on participant-aggregated ratings
($N=285$). Bold values indicate the dominant loading for each item. Parallel analysis
used 10,000 simulated datasets; factors were retained when the observed eigenvalue
exceeded the 95th-percentile random eigenvalue.}
\label{tab:efa_parallel}

\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
% \toprule
& \multicolumn{2}{c}{\textbf{EFA loadings}}
& \multicolumn{5}{c}{\textbf{Parallel analysis}} \\

\cmidrule(lr){2-3}
\cmidrule(lr){4-8}

\textbf{Evaluation item}
& \textbf{F1}
& \textbf{F2}
& \textbf{Factor}
& \textbf{Observed}
& \textbf{Random mean}
& \textbf{Random 95\%}
& \textbf{Retain} \\
\midrule

Readability
& \textbf{.735} & -.079
& 1 & 6.020 & 1.304 & 1.390 & Yes \\

Reasoning clarity
& \textbf{.879} & .022
& 2 & 1.423 & 1.210 & 1.271 & Yes \\

\hdashline
Situational fit
& \textbf{.800} & -.080
& 3 & .706 & 1.138 & 1.187 & No \\
Risk acknowledgement
& \textbf{.553} & .245
& 4 & .616 & 1.076 & 1.119 & No \\
\hdashline

Financial harm risk
& -.132 & \textbf{.654}
& 5 & .432 & 1.019 & 1.059 & No \\

Misleadingness
& .019 & \textbf{.819}
& 6 & .271 & .965 & 1.004 & No \\
\hdashline

Perceived source knowledge
& \textbf{.899} & .110
& 7 & .232 & .911 & .952 & No \\

Overall quality
& \textbf{.942} & .019
& 8 & .151 & .855 & .899 & No \\
\hdashline

Trust intention
& \textbf{.883} & -.069
& 9 & .097 & .797 & .845 & No \\

Reliance intention
& \textbf{.881} & -.074
& 10 & .052 & .727 & .783 & No \\

\bottomrule
\end{tabular}
}
\end{table}

==> tables/9_qtr_results.tex <==
% Table: Evaluation pathway to quality, trust, and reliance
\begin{table*}[t]
\centering
\sffamily

\caption{Mixed-effects models of downstream advice evaluation.
Coefficients are standardized fixed-effect estimates ($\beta$). Each column represents the fully adjusted model for the corresponding downstream judgment.}
\label{tab:evaluation-pathway}

\setlength{\tabcolsep}{13pt}
\renewcommand{\arraystretch}{1.22}

\begin{tabular}{lccc}
\toprule
&
\textbf{Overall Quality} &
\textbf{Trust} &
\textbf{Reliance} \\
\midrule

\multicolumn{4}{l}{\textit{Initial advice appraisals}} \\
\addlinespace[0.15em]

Message Appraisal
& \posthree{+0.325***}
& \posthree{+0.132***}
& \posthree{+0.079***} \\

Risk Acknowledgement
& \posthree{+0.075***}
& +0.024
& -0.015 \\

Safety Concern$^\dagger$
& \negthree{-0.088***}
& \negthree{-0.125***}
& \negthree{-0.050***} \\

Source Knowledge
& \posthree{+0.489***}
& \posthree{+0.109***}
& \posone{+0.047*} \\

\addlinespace[0.45em]
\multicolumn{4}{l}{\textit{Downstream evaluations}} \\
\addlinespace[0.15em]

Overall Quality
& ---
& \posthree{+0.607***}
& \posthree{+0.206***} \\

Trust
& ---
& ---
& \posthree{+0.594***} \\

\addlinespace[0.25em]
\midrule

\multicolumn{4}{l}{\textit{Model fit}} \\
\addlinespace[0.10em]

Marginal $R^2$: upstream model
& 0.098 & 0.112 & 0.148 \\

Conditional $R^2$: upstream model
& 0.373 & 0.351 & 0.362 \\[0.15em]

Marginal $R^2$: evaluation model
& \textbf{0.692}
& \textbf{0.759}
& \textbf{0.829} \\

Conditional $R^2$: evaluation model
& 0.742
& 0.795
& 0.829 \\

\bottomrule
\end{tabular}

\vspace{0.5em}

\begin{minipage}{0.92\textwidth}
\footnotesize
\textit{Note.}
$N=1{,}140$ evaluations from 285 participants.
All models include participant random intercepts and adjust for advice communication
style, displayed source attribution, stakes, external uncertainty, verifiability, and
scenario familiarity. $R^2_m$ denotes marginal $R^2$ (fixed effects); $R^2_c$ denotes
conditional $R^2$ (fixed and random effects).
$^{*}p<.05$, $^{**}p<.01$, $^{***}p<.001$.
\end{minipage}

\end{table*}
